A Parallel Distributed Strategy for Arraying a Scattered Robot Swarm

We consider the problem of organizing a scattered group of $n$ robots in two-dimensional space, with geometric maximum distance $D$ between robots. The communication graph of the swarm is connected, but there is no central authority for organizing it. We want to arrange them into a sorted and equally-spaced array between the robots with lowest and highest label, while maintaining a connected communication network. In this paper, we describe a distributed method to accomplish these goals, without using central control, while also keeping time, travel distance and communication cost at a minimum. We proceed in a number of stages (leader election, initial path construction, subtree contraction, geometric straightening, and distributed sorting), none of which requires a central authority, but still accomplishes best possible parallelization. The overall arraying is performed in $O(n)$ time, $O(n^2)$ individual messages, and $O(nD)$ travel distance. Implementation of the sorting and navigation use communication messages of fixed size, and are a practical solution for large populations of low-cost robots.

==> Makefile <==
LANGUAGE = en_US
DOCUMENTS = main.pdf
TEXFILES := $(sort $(wildcard *.tex))

PDFLATEX = pdflatex
PDFLATEXFLAGS = -halt-on-error -file-line-error
BIBTEX = bibtex
BIBTEXFLAGS =

#GRAPHICS_STATIC = $(foreach g, \
#	prototyp.pdf, \
#	pics/$g)

GRAPHICS_STATIC =

GRAPHICS_PDF =

GRAPHICS_PDFTEX = $(foreach g, \
	3sat gadget_and gadget_crossing gadget_inverter gadget_multiplexer \
	gadget_or_bb gadget_or_rb gadget_variable needles three_colorability, \
	graphics/$g.pdf_tex)

main.pdf: main.tex ieeeconf.cls 01-Introduction.tex 02-ModelAndPreliminaries.tex 03-Alg.tex 03X-Sorting.tex 04-Implementation.tex 05-Simulation.tex 06-Conclusion.tex mclurkin.bib lit.bib 
#	$(GRAPHICS_STATIC) $(GRAPHICS_PDF) $(GRAPHICS_PDFTEX)

.DEFAULT_GOAL = all
.PHONY: all todo spellcheck clean

all: $(DOCUMENTS)

todo:
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		grep -hnT TODO $$texfile || true; \
		grep -hnTo '\\\(todo\|missingfigure\)\(\[.*\]\)\?{.*}' $$texfile | detex || true; \
	done

spellcheck:
	for texfile in $(TEXFILES); do \
		aspell --lang=$(LANGUAGE) check $$texfile; \
	done

$(DOCUMENTS): %.pdf: %.tex
	$(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}
	if grep -e '\citation' -e '\bibdata' -e '\bibstyle' *.aux; then \
		$(BIBTEX) $(BIBTEXFLAGS) $* && $(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}; \
	fi
	$(PDFLATEX) $(PDFLATEXFLAGS) -recorder \\input{$<}
	grep '^OUTPUT ' $*.fls \
		| sed -e 's/^OUTPUT //' \
		| grep -vx $@ \
		| xargs rm
	rm $*.fls
	rm -f $*.bbl $*.blg

%.ps: %.pdf
	pdf2ps -dLanguageLevel=3 $< $@

$(GRAPHICS_PDF): %.pdf: %.svg
	inkscape --without-gui --export-pdf=$*.pdf $*.svg

$(GRAPHICS_PDFTEX): %.pdf_tex: %.svg
	inkscape --without-gui --export-latex --export-pdf=$*.pdf $*.svg

clean:
	rm -f $(DOCUMENTS)
	rm -r main.pdf
	rm -f *.aux *.bbl *.blg *.log *.out 
#	rm -f $(GRAPHICS_PDF)
#	rm -f $(GRAPHICS_PDFTEX)
#	rm -f $(GRAPHICS_PDFTEX:.pdf_tex=.pdf)

